Fully Dynamic $(1+\epsilon)$-Approximate Matchings

We present the first data structures that maintain near optimal maximum cardinality and maximum weighted matchings on sparse graphs in sublinear time per update. Our main result is a data structure that maintains a $(1+\epsilon)$ approximation of maximum matching under edge insertions/deletions in worst case $O(\sqrt{m}\epsilon^{-2})$ time per update. This improves the 3/2 approximation given in [Neiman,Solomon,STOC 2013] which runs in similar time. The result is based on two ideas. The first is to re-run a static algorithm after a chosen number of updates to ensure approximation guarantees. The second is to judiciously trim the graph to a smaller equivalent one whenever possible. We also study extensions of our approach to the weighted setting, and combine it with known frameworks to obtain arbitrary approximation ratios. For a constant $\epsilon$ and for graphs with edge weights between 1 and N, we design an algorithm that maintains an $(1+\epsilon)$-approximate maximum weighted matching in $O(\sqrt{m} \log N)$ time per update. The only previous result for maintaining weighted matchings on dynamic graphs has an approximation ratio of 4.9108, and was shown in [Anand,Baswana,Gupta,Sen, FSTTCS 2012, arXiv 2012].

==> lazy_long.tex <==
\section{$(1 + \epsilon)$-MCMs Using Lazy Updates}
%\section{Laziness and Approximate Matchings}
\label{sec:lazy}

In this section we will use the algorithm previously 
developed to design another algorithm that maintains
a $(1 + \epsilon)$-MCM in $O(m / \epsilon^{2})$ time
per update.
Our starting point is the observation that the size of maximum
matching changes by at most $1$ per update.
This means that if we have a large matching that's close to
the maximum, it will remain close over a large number of updates.
To simplify the presentation for the rest of this section,
we number the updates from $1$ to $t$.
We will use $G_i$ to denote the graph after the ith update,
and use $\optmatchingsize{i}$ to denote the size of the
maximum matching in $G_i$.
Note that due to edge deletions, a matching $M_i$ computed for
$G_i$ might not be a valid matching in $G_j$.
However, we can restrict it to a matching in $G_j$ by removing
the deleted edges, and we will denote this as $M_i(j)$.
This simple fact can be formalized as follows:

\begin{lemma}
\label{lem:stable}
If $M$ is an $(1 + \epsilon)$-MCM in $G_i$,
then for $j = i + \epsilon |M|$,
$M(j)$ is an $(1 + \epsilon + \epsilon')$-MCM in $G_{j}$
\end{lemma}

\begin{proof}
Suppose there were $k_+$ insertions and $k_-$ deletions in
the $k=\epsilon' |M|$ updates between updates $i$ and $j$.
The assumption about $M$ gives that $\optmatchingsize{i}
\leq (1 + \epsilon) |M|$.
Since each insert can increase the size of the maximum
matching by $1$, we have
$|\optmatchingsize{j}| \leq |\optmatchingsize{i}|+ k_i$.
Also, each deletion can remove at most one edge from $M$,
so $|M(j)| \geq |M| - k_d$.
The approximation ratio is then at most:
\begin{align}
\frac{\optmatchingsize{i}}{|M(j)|}
\leq & \frac{(1 + \epsilon) |M| + k_i}{|M| - k_d} \nonumber\\
= & 1 + \frac {\epsilon |M| + k }{|M|-k_d} \nonumber \\
\leq & 1 + \frac{\epsilon |M| + \epsilon' |M|} {|M|} \nonumber \\
\leq & 1 + \epsilon + \epsilon'
\end{align}
\end{proof}

This fact has immediate algorithmic consequences for situations
where the maximum matching is large.
Suppose we computed an $1 + \epsilon / 2$-MCM for $G_i$, $M_i$,
then we can use $M_i(j)$ as long as $j \leq i + \epsilon |M_i| / 2$.
The $O(m / \epsilon)$ cost of the call to \textsc{ApproxMCM}
(given by Lemma \ref{lem:static}) can then be chanrged to the
towards the next $\epsilon |M_i| / 2$ updates, giving
$O(m / |M_i| / \epsilon^2)$ charged per update.
In case of large values of $|M_i|$, this cost is fairly small,
but for small values such as constant sized $|M_i|$, we are
still making a call to \textsc{ApproxMCM} almost every update.

One more idea is needed to reduced the cost of such a call when
$|M_i|$ is small.
For this, we turn to a key idea from Section \ref{sec:twothirds},
which is to consider a small subset of the vertices as special.
Our choice of these vertices stems from a cruicial step in the
data structure by Onak and Rubinfield \cite{onak2010maintaining}.
The observation that they used is that small maximum matchings
also implies small vertex covers.
In other words, all edges in the graph contain at least one end
point in a small set of vertices $C$.


This observation can allow us to find matchings on a much smaller
graph built from this vertex cover.
\begin{lemma}
\label{lem:smallcover}
Let $C \subseteq V$ be a vertex cover, and $G'$ be a graph consisting of:
\begin{itemize}
\item All edges between vertices in $C$
\item Up to $|C|$ arbitrary edges to vertices in $V \setminus C$
for each vertex in $C$.
\end{itemize}
If $M'$ is a $1 + \epsilon$-MCM in $G'$, then it's
also a $1 + \epsilon$-MCM in $G$.
\end{lemma}

\begin{proof}
We first show that the size of the maximum matching in $G$
is the same as the size of the maximum matching in $G'$
by contradiction.
Among all maximum matchings in $G$, let
$M$ be one that uses the maximum number of edges in $E(G')$.
Suppose $M$ is not contained in $E(G')$, then
it contains an edge $(u, v)$ in $E(G) \setminus E(G')$.
Since $C$ is a vertex cover, one of $u$ or $v$ is in $C$,
without loss of generality assume it's $u$.
%As all edges between vertices of $C$ are kept,
%we may assume that $v \notin S$.
Since $(u, v) \notin G'$, there are $|C|$ neighbors of $u$
that are kept in $G'$, let them be $N_{V \setminus C}(u)$.
As the maximum matching in $G$ has size at most $|C|$,
and $v \notin N_{V \setminus C}(u)$, there are at most
$|C| - 1$ edges in $M$ involving a vertex in $N_{V \setminus C}(u)$.
Therefore there exists $w \in C \setminus G$ such that $(u, w) \in G'$
and $(u, w) \notin M$.
Substituting $(u, v)$ with $(u, w)$ gives a maximum matching
that uses one more edge in the $G'$, giving a contradiction.

Since $E(G') \subseteq E(G)$, $M$ is also a matching in $G$.
As the size of the maximum matchings in these two graphs are
the same, $M$ is also a $1 + \epsilon$-MCM in $G$. 
\end{proof}

This vertex cover $C$ can be obtained by taking all vertices
involved in a maximal matching.
As a maximal matching has size at most $(1 + \epsilon)|M_i|$,
$|C|$ has size at most $2(1 + \epsilon)|M_i| \leq O(|M_i|)$.
Therefore in the case that $|M_i|$ is small,
we only need to run the static algorithm given by Lemma
\ref{lem:static} on a graph with $O(|M_i|^2)$ edges.
Assuming we have access to $C$, constructing this graph
can be done time linear to the size of $G'$.
So instead of charging $O(m / \epsilon)$ to the next $\epsilon / 2|M_i|$
udpates, we can charge $O(|M_i|^2 /\epsilon)$ instead.
Therefore, the cost charged to each such update is
$O(|M_i| / \epsilon^2)$, which is small for small values of $|M_i|$.
Adding this trimming of the graph in the algorithm allows us to
give our data structure for maintaining $1 + \epsilon$-MCMs
with low amortized costs.

Our data structure maintains the following global states:
\begin{enumerate}
	\item The current graph $G$, stored as a doubly linked list.
	\item A matching $M$.
	\item A counter $t$ indicating the number of updates until we make the next call
	\item A vertex cover with size $O(|M|)$.
\end{enumerate}

Upon initialization $M$ is obtained by running the static
algorithm on $G$, or can be set to $\empty$ if $G$ starts empty.
To maintain the vertex cover, we use our algorithm which
maintains 3/2-approximate matching from Section \ref{sec:twothirds}
and output its matched vertices as the vertex cover.
This takes $O(\sqrt m)$ time per update, which is less than our bound.
As the cost of constructing $G'$ is significantly more than
accessing $|C|$, we will assume oracle access to the cover for the
rest of this section.
As we handle insertions and deletions in almost symmetrical
ways, we present them as a single routine $\textsc{Update}$,
shown in Figure \ref{fig:lazy}

\begin{figure}[ht]
\begin{procedure}[H]
	\nl Update the Doubly Linked List Representing $G$ to Reflect Changes \;
	\nl \If{Update is a deletion and $(u,v) \in M$}{
		\nl Remove $(u, v)$ from $M$\;
	}
	\nl $t \leftarrow t - 1$ \;
	\nl \If{$t \leq 0$}{
		\nl Construct graph $G'$ by taking all edges within $C$, along with first $|C|$ neighbors in $V \setminus C$ of each vertex in $C$ \;
		\nl $M \leftarrow \textsc{ApproxMCM}(G', 1 + \epsilon / 2)$ \;
		\nl $t \leftarrow |M|$ \;
	}
\caption{UPDATE(u,v)}
\end{procedure}
\caption{Lazy update algorithm for maintaining $1 + \epsilon$-MCMs}
\label{fig:lazy}
\end{figure}

The bounds of this routine is as follows:

\begin{theorem}
\label{thm:lazy}
The matching $M$ is an $(1 + \epsilon)$-MCM over all updates.
Furthermore, the amortized cost per update is $O(m^{1/2} / \epsilon^2)$.
\end{theorem}


\begin{proof}
The guarantees of the size of $M$ follows from Lemma \ref{lem:stable}.

For running time, let the current update be at time $j$, and the
$M$ that we maintained was found in iteration $i < j$, aka
$M = M_i(j)$.
Note that we cannot really charge the cost of the
call to the next $|M_j|$ iteraitons since those iteraitons might not
take place.
Instead we charge them updates numbered from $i + 1$ to $j$.
Note that $M_i(j - 1)$ was a $1 + \epsilon$ MCM for $G_{j - 1}$,
so $\optmatchingsize{i} \leq (1+\epsilon)|M_i| + 1 \leq O(|M_i| + 1)$.
Therefore $|E(G_j')| \leq O(\min \{ m, (|M_i|+1)^2 \} )$, and the
total cost of constructing $G'_j$ and running \textsc{ApproxMCM}
on it can be bounded by $O(\min \{ m, (|M_i|+1)^2 \} / epsilon)$.

By the choice of $t$, $j - i = \max{1, \epsilon / 2 |M_i|}$.
In the later case, the cost charged to update $i$ is $O(1)$,
while in the former the cost is:
\begin{align*}
\frac{O(\min \{ m, (|M_i|+1)^2 \} / \epsilon)}{\epsilon / 2 |M_i|}
= O( \min \{ \frac{m}{|M_i|}, |M_i| \} / \epsilon^2 )
\end{align*}
If $|M_i| \geq \sqrt{m}$, the first term inside $\min$ is at most
$\sqrt{m}$, otherwise the second is at most $\sqrt{m}$.
Combining these two cases gives our desired bound.
\end{proof}


The worst case cost of each call to \textsc{Update}
in this scheme is still $O(m / \epsilon)$ due to the call to
$\textsc{ApproxMCM}$.
However, Lemma \ref{lem:stable} gives that in this case, the matching
will remain an $(1 + 2 \epsilon)-MCM$ after $\epsilon |M|$ updates.
As a result, this call can take place in a more gradual fashion,
and be spread over the next $\epsilon |M|$ updates.
This call can in fact be used as a way to time the start of the
next call to \textsc{ApproxMCM}.
As the construction of $G'$ can also be expensive, it is helpful
to view finding it, and running $\textsc{ApproxMCM}$ on it
as a single round.
This leads to an even simpler, and lazier algorithm where the
start of the next round is timed by the completion of
the current one.
Pseudocode of this algoirthm is shown in Figure \ref{fig:lazyworst}.

\begin{figure}[ht]
\begin{procedure}[H]
	\nl Update the Doubly Linked List Representing $G$ to Reflect Changes \;
	\nl \If{Update is a deletion and $(u,v) \in M$}{
		\nl Remove $(u, v)$ from $M$\;
	}
	\nl Perform $O(\sqrt{m} / \epsilon^2)$ steps in the current round\;
	\nl \If{Current round finishes}{
		\nl Replace $M$ by the result of this call with deleted edges removed.
		\nl Initiate the next round consisting of the construction of $G'$, and $\textsc{ApproxMCM}(G', 1 + \epsilon / 4)$ \;
	}
\caption{UPDATEGRADUAL(u,v)}
\end{procedure}
\caption{Maintaining $1 + \epsilon$-MCMs with Worst Case Guarantees}
\label{fig:lazyworst}
\end{figure}

In order to analyze this algorith, we first prove some properties of
the way it times itself.
We relate the number of updates it takes for a call initiated at update
$i$ to finish with the value of $\optmatchingsize{i}$ using a proof
analogous to that of Theorem \ref{thm:lazy}

\begin{lemma}
\label{lem:singlecall}
If a call to \textsc{ApproxMCM} initiated at update $i$
is ran for $O(\sqrt{m} / \epsilon^2)$ steps per update for
a right constant, it will finish within $\epsilon/8 \optmatchingsize{i}$
updates.
\end{lemma}

\begin{proof}
By the same argument as before, the size of $C$ is at most
$\optmatchingsize{i}$, and the number of edges in $G'$ can be bounded
by $O(\min\{m, \optmatchingsize{i}^2 \})$.
This means that the total cost of the current round is 
$O(\min\{m, \optmatchingsize{i}^2 \} / \epsilon)$.
For this to finish in $\epsilon / 8 \optmatchingsize{i}$ updates,
the amount of work that needs to be performed at each update is:
\begin{align*}
	O(\min\{\frac{m}{\optmatchingsize{i}}, \optmatchingsize{i} \} / \epsilon^2)
\end{align*}
A $O(\sqrt{m} / \epsilon^2)$ bound on work needed per update
can then be obtained by considering cases of $\optmatchingsize{i} \geq \sqrt{m}$
and $\optmatchingsize{i} < \sqrt{m}$.
\end{proof}

The worst case bounds can now be obtained by analyzing the duration
for which $M_i(j)$ is used as $M$ in the algorithm.

\begin{theorem}
\label{thm:stable}
The lazy update algorithm runs in  $O(\sqrt{m} / \epsilon^2)$ per update,
and at any point $M$ is an $(1 + \epsilon)$-MCM
\end{theorem}

\begin{proof}
The running time follows from the limit on the number of steps
of \textsc{ApproxMCM} ran per call, and Theorem \ref{thm:twothirdworstcase}
For the guarantees on $M$, it suffices to prove that the matching
produced by a round initiated at update $i$ remains an
$1 + \epsilon$-MCM until the completion of the next round.

Let $M_i$ be a matching produced by a round initiated at update $i$.
Assume it is returned at the start of update $i'$.
Lemma \ref{lem:singlecall} gives:
\begin{align*}
i' \leq i + \epsilon/8 \optmatchingsize{i}
\end{align*}
and that the round initiated at update $i'$ finishes 
in $\epsilon / 8 \optmatchingsize{i'}$ updates.
Therefore it suffices to show that $M_i(j)$ is a $1 + \epsilon$-MCM
for $G_j$ for all $j \leq i +
\epsilon/8 (\optmatchingsize{i} + \optmatchingsize{i'})$.

Since the call to \textsc{ApproxMCM} is ran with error $\epsilon / 4$,
we have $\optmatchingsize{i} \leq (1 + \epsilon / 4) |M_i|$,
and:
\begin{align}
\optmatchingsize{i'}
\leq & \optmatchingsize{i} + (i' - i) \nonumber\\
\leq & (1 + \epsilon / 8) \optmatchingsize{i} \nonumber\\
\leq & (1 + \epsilon / 8) (1 + \epsilon / 4) |M_i|
\end{align}
Summing these then gives:
\begin{align}
\epsilon/8 (\optmatchingsize{i} + \optmatchingsize{i'})
\leq & \epsilon / 8 ((1 + \epsilon / 4) |M_i| + (1 + \epsilon / 8) (1 + \epsilon / 4) |M_i|) \nonumber\\
= & \epsilon / 8 (2 + \epsilon / 8) (1 + \epsilon / 4) |M_i| \nonumber\\
\leq & 3\epsilon / 4 |M_i|
\end{align}
The bounds then follows from \ref{lem:stable} with
$\epsilon' = 3 \epsilon / 4$.
\end{proof}



==> worstcase.tex <==
\section{Achieving worst case $O(\sqrt  m )$ update time}
\label{sec:worst}

\paragraph*{Dirty Phase}

Once the value of \m D changes, a number of vertices may be at an incorrect level, depending on their degree and 
the value of \m D. A way to solve this problem is to examine each vertex and move it to the correct level if it
is not at one. But this may take $O(m)$ time and hence the amortization factor is introduced by spreading this
cost over several updates.
To avoid the amortization factor, we do not correct the levels of all the vertices once the value of \m D changes.
But if all the vertices are not at their correct level then the first invariant is violated. We term a situation
in which all vertices do not satisfy the first invariant of the algorithm a `dirty' phase.
Thus, a change in value of \m D, begins a `dirty' phase. This phase ends when all the vertices in the graph
satisfy the first invariant. 

We use a strategy such that the dirty phase ends before the next change in value of \m D occurs.
Whenever a change in value of \m D occurs there may be some vertices at level $1$ which should actually be at
level $0$ or there may be some vertices at level $0$ which should actually be at level $0$. Note that the new value
of \m D is within a constant factor of the old value of \m D and hence the vertices who actually have to move from
level $0$ to $1$ or vice-versa have degree $O(\sqrt m)$. Specifically, the value of \m D may change from $3\sqrt m$ to
$4\sqrt m$ or from $5\sqrt m$ to $4\sqrt m$. Thus, the vertices which will have to move between levels have degree
between $3 \sqrt m$ to $4\sqrt m$ or between $4\sqrt m$ to $5\sqrt m$. In any case their degree is $O(\sqrt m)$. Their
degrees will remain $O(\sqrt m)$, where $m$ is the current number of vertices in the graph, at least until
the next change in value of \m D occurs. 

\paragraph*{Ending dirty phase before next change in \m D occurs}

Every edge update involves
two vertices, the end points of the edge being added or deleted. Whenever an update occurs we check for the two
vertices involved that if they are not at the correct level they are moved to the correct level. To actually end the
dirty phase, we need a mechanism to check all the vertices if they are at the right level or not. To do this we
maintain a set of vertices having degree at least one. Note that this set of vertices has a size $\leq m +  1$.
If we keep on checking a constant number of vertices in each update then we can check all the vertices before the
change in \m D occurs next, provided we choose that constant appropriately.

Suppose when the value of \m D is set the number of edges is $m$. Using calculations in Lemma $4$, we can see that
the next change in value of \m D occurs at least $\frac{9m}{25}$ updates later. And the number of vertices which
have to be checked is $< 2m$. So, we can check $\frac{2m}{9m/25}$ vertices after every update and we will be sure
that the dirty phase ends before the next change in value of \m D occurs. We can pick any constant number
greater than $\frac{50}{9}$ and so the number of vertices to be
checked after every update is picked to be $8$. So, after the $k^{th}$ update in the dirty phase we check $(8(k - 1) + 1)^{th}$
vertex to $8k^{th}$ vertex in the set of vertices having degree greater than $1$. After we check all the vertices
the dirty phase ends. Since we have chosen the number of vertices checked in a particular way, the dirty phase ends
before the next change in \m D occurs. 

As the degree of vertices which move have $O(\sqrt m)$ degree, we incur an extra cost
of $O(8 \sqrt m )$ which is $O(\sqrt m )$ per update in the dirty phase. This does not increase the time complexity of the
algorithm executed after every update.
We can now state the following theorem -

\begin{theorem}
\label{thm:twothirdworstcase}
There exists a deterministic fully dynamic worst case $O(\sqrt m )$ update time algorithm for maintaining 
$\frac{3}{2}$ approximate maximum cardinality matching.
\end{theorem}





